A Uniform Framework for Handling Position Constraints in String Solving (Technical Report)

We introduce a novel decision procedure for solving the class of position string constraints, which includes string disequalities, not-prefixof, not-suffixof, str$.$at, and not-str$.$at. These constraints are generated frequently in almost any application of string constraint solving. Our procedure avoids expensive encoding of the constraints to word equations and, instead, reduces the problem to checking conflicts on positions satisfying an integer constraint obtained from the Parikh image of a polynomial-sized finite automaton with a special structure. By the reduction to counting, solving position constraints becomes NP-complete and for some cases even falls into PTime. This is much cheaper than the previously used techniques, which either used reductions generating word equations and length constraints (for which modern string solvers use exponential-space algorithms) or incomplete techniques. Our method is relevant especially for automata-based string solvers, which have recently achieved the best results in terms of practical efficiency, generality, and completeness guarantees. This work allows them to excel also on position constraints, which used to be their weakness. Besides the efficiency gains, we show that our framework may be extended to solve a large fragment of not-contains (in NExpTime), for which decidability has been long open, and gives a hope to solve the general problem. Our implementation of the technique within the Z3-Noodler solver significantly improves its performance on position constraints.

==> tables/solved.tex <==
\begin{booktabs}{colspec={lQ[r,gray!30]Q[r,gray!30]Q[r,gray!30]rrrQ[r,gray!30]Q[r,gray!30]Q[r,gray!30]rrrQ[r,gray!30]Q[r,gray!30]Q[r,gray!30]},rowsep=0pt,row{4}={yellow},cell{1,2}{2,5,8,11,14}={c=3}{c}}
    \toprule
    &  \biopython & & & \django & & & \thefuck & & & \poshard & & & All & & \\
    &  (77,222)     & & & (52,643)   & & & (19,872)    & & & (550)    & & & (150,287) & & \\
    \cmidrule[lr]{2-4}\cmidrule[lr]{5-7}\cmidrule[lr]{8-10}\cmidrule[lr]{11-13}\cmidrule[lr]{14-16}
    & \oob & \unknown & \timet & \oob & \unknown & \timet & \oob & \unknown & \timet & \oob & \unknown & \timet & \oob & \unknown & \timet \\
    \midrule
    \ziiinoodlerpos & 171    & 0     & 3,490     & 39     & 0      & 3,325      & 0     & 0       & 665        & 0     & 0       &  124    & 210    & 0       & 7,605 \\
    \ziiinoodler    & 171    & 336   & 3,545     & 37     & 108    & 3,473      & 1     & 375     & 637        & 234   & 246     & 1,912   & 443    & 1,065   & 9,567 \\
    \cvcv           & 69     & 0     & 12,834    & 0      & 0      & 4,515      & 0     & 0       & 690        & 550   & 0       & --      & 619    & 0       & 18,040 \\
    \ziii           & 1,047  & 0     & 15,661    & 502    & 0      & 7,501      & 47    & 0       & 9,457      & 550   & 0       & --      & 2,146  & 0       & 32,620 \\
    \ostrich        & 2,986  & 0     & 749,986   & 4,404  & 0      & 979,326    & 967   & 0       & 120,152    & 550   & 0       & --      & 8,907  & 0       & 1,849,465 \\
    \bottomrule
    \end{booktabs}
    
